Parameter Interpolation Adversarial Training for Robust Image Classification

Though deep neural networks exhibit superior performance on various tasks, they are still plagued by adversarial examples. Adversarial training has been demonstrated to be the most effective method to defend against adversarial attacks. However, existing adversarial training methods show that the model robustness has apparent oscillations and overfitting issues in the training process, degrading the defense efficacy. To address these issues, we propose a novel framework called Parameter Interpolation Adversarial Training (PIAT). PIAT tunes the model parameters between each epoch by interpolating the parameters of the previous and current epochs. It makes the decision boundary of model change more moderate and alleviates the overfitting issue, helping the model converge better and achieving higher model robustness. In addition, we suggest using the Normalized Mean Square Error (NMSE) to further improve the robustness by aligning the relative magnitude of logits between clean and adversarial examples rather than the absolute magnitude. Extensive experiments conducted on several benchmark datasets demonstrate that our framework could prominently improve the robustness of both Convolutional Neural Networks (CNNs) and Vision Transformers (ViTs).

==> Figure/ALP_NMSE.tex <==
\begin{table}[t]
\caption{The clean and robust accuracy (\%) of NMSE and ALP under adversarial attacks on CIFAR10 and CIFAR100 datasets with ResNet18 model.}
\label{tab: ALP_NMSE}
\centering
\begin{center}
\begin{small}
% \begin{sc}
\begin{tabular}{cccccccc}
\toprule
Dataset & Method &Clean & PGD20 & AA \\
\midrule
\multirow{2}*{CIFAF10}
&ALP&79.74&\textbf{52.37}&46.13\\
&\textbf{NMSE}&\textbf{84.77}&51.56&\textbf{46.60}\\
\midrule
\multirow{2}*{CIFAF100}
&ALP&57.29&28.12&23.57\\
&\textbf{NMSE}&\textbf{58.88}&\textbf{29.55}&\textbf{24.82}\\
\bottomrule
\end{tabular}
% \end{sc}
\end{small}
\end{center}
\end{table}

==> Figure/Decision_Boundary_PGDAT_PIAT.tex <==
\begin{figure*}[t]
    \centering
    \subcaptionbox{The initial decision boundary before the 20\(^{th}\) epoch of PGD-AT\label{PGDAT:a}}{
    \includegraphics[width=0.225\textwidth]{Figure/Boundary_19.pdf}}
    \subcaptionbox{The final decision boundary after the 20\(^{th}\) epoch of PGD-AT\label{PGDAT:b}}{
    \includegraphics[width=0.225\textwidth]{Figure/Boundary_20.pdf}}
    \subcaptionbox{The initial decision boundary before the 21\(^{th}\) epoch of PIAT\label{PIAT:a}}{
    \includegraphics[width=0.225\textwidth]{Figure/PIAT_boundary_20.pdf}}
    \subcaptionbox{The final decision boundary after the 21\(^{th}\) epoch of PIAT\label{PIAT:b}}{
    \includegraphics[width=0.225\textwidth]{Figure/PIAT_boundary_21.pdf}}
    \caption{The decision boundary change of model trained by PGD-AT and PIAT when model robustness exhibit a sudden decrease.
    }
    \label{fig:Decision Boundary of PGDAT and PIAT}
\end{figure*}

==> Figure/Hyperparameter_NMSE.tex <==
\begin{figure}[t]
% \vspace{-1.0em}
    \centering
    {
    \includegraphics[width=0.44\textwidth]{Figure/Hyperparameter_NMSE_CIFAR10.pdf}}
    \caption{The clean and robust accuracy (\%) on CIFAR10 dataset for different hyper-parameters of the NMSE regularization term when combined with the \name framework. The performance of NMSE indicates that it is not sensitive to hyper-parameter \(\mu\).
    }
    \label{fig:Hyperparameter of NMSE}
\end{figure}

==> Figure/Motivation.tex <==
\begin{figure*}[t]
    \centering
    \subfigure[The decision boundary before the 27\(^{th}\) epoch of PGD-AT\label{subfig:a}]{
    \includegraphics[width=0.45\textwidth]{Figure/Boundary_26.pdf}}
    \subfigure[The decision boundary after the 27\(^{th}\) epoch of PGD-AT\label{subfig:b}]{
    \includegraphics[width=0.45\textwidth]{Figure/Boundary_27.pdf}}
    \caption{
    The 2D decision boundary of model trained by PGD-AT in the 27\(^{th}\) epoch.
    while the blue data points around the top left of decision boundary are correctly classified, the red data points around the top left and right of decision boundary are misclassified.
    }
    \label{fig:Decision Boundary}
\end{figure*}

==> Figure/PGDAT_decision_boundary.tex <==
\begin{figure*}[t]
\vspace{-1em}
    \centering
    % \subfigure{The initial decision boundary before the 20\(^{th}\) epoch of PGD-AT\label{PGDAT:12}}{
    % \includegraphics[width=0.225\textwidth]{Figure/Boundary_12.pdf}}
    % \subfigure{The final decision boundary after the 20\(^{th}\) epoch of PGD-AT\label{PGDAT:13}}{
    % \includegraphics[width=0.225\textwidth]{Figure/Boundary_13.pdf}}
    % \subfigure[Before the 12\(^{th}\) epoch\label{PGDAT:11}]{
    % \includegraphics[width=0.225\textwidth]{Figure/Boundary_11.pdf}}
    % \subfigure[After the 12\(^{th}\) epoch\label{PGDAT:12}]{
    % \includegraphics[width=0.225\textwidth]{Figure/Boundary_12.pdf}}
    % \subfigure[Before the 14\(^{th}\) epoch\label{PGDAT:13}]{
    % \includegraphics[width=0.225\textwidth]{Figure/Boundary_13.pdf}}
    % \subfigure[After the 14\(^{th}\) epoch\label{PGDAT:14}]{
    % \includegraphics[width=0.225\textwidth]{Figure/Boundary_14.pdf}}
    % \subfigure[Before the 20\(^{th}\) epoch\label{PGDAT:19}]{
    % \includegraphics[width=0.225\textwidth]{Figure/Boundary_19.pdf}}
    % \subfigure[After the 20\(^{th}\) epoch\label{PGDAT:20}]{
    % \includegraphics[width=0.225\textwidth]{Figure/Boundary_20.pdf}}
    % \subfigure[Before the 27\(^{th}\) epoch\label{PGDAT:26}]{
    % \includegraphics[width=0.225\textwidth]{Figure/Boundary_26.pdf}}
    % \subfigure[After the 27\(^{th}\) epoch\label{PGDAT:27}]{
    % \includegraphics[width=0.225\textwidth]{Figure/Boundary_27.pdf}}
    % \subfigure[Before the 31\(^{th}\) epoch\label{PGDAT:30}]{
    % \includegraphics[width=0.225\textwidth]{Figure/Boundary_30.pdf}}
    % \subfigure[After the 31\(^{th}\) epoch\label{PGDAT:31}]{
    % \includegraphics[width=0.225\textwidth]{Figure/Boundary_31.pdf}}
    % \subfigure[Before the 34\(^{th}\) epoch\label{PGDAT:33}]{
    % \includegraphics[width=0.225\textwidth]{Figure/Boundary_33.pdf}}
    % \subfigure[After the 34\(^{th}\) epoch\label{PGDAT:34}]{
    % \includegraphics[width=0.225\textwidth]{Figure/Boundary_34.pdf}}
    \subfigure[From 13\(^{th}\) to 14\(^{th}\) epoch\label{PGDAT:14}]{
    \includegraphics[width=0.35\textwidth]{Figure/Boundary_13_14.pdf}}
    \subfigure[From 19\(^{th}\) to 20\(^{th}\) epoch\label{PGDAT:20}]{    \includegraphics[width=0.35\textwidth]{Figure/Decision Boundary 26-27.pdf}} \\
    \vspace{-1.2em}
    \subfigure[From 26\(^{th}\) to 27\(^{th}\) epoch\label{PGDAT:27}]{
    \includegraphics[width=0.35\textwidth]{Figure/Boundary_33_34.pdf}}
    \subfigure[From 33\(^{th}\) to 34\(^{th}\) epoch\label{PGDAT:34}]{
    \includegraphics[width=0.35\textwidth]{Figure/PIAT_boundary_17_18.pdf}}
    \vspace{-1em}
    \caption{
    % The initial/final decision boundary of PIAT before/after an epoch when the model robustness exhibits a sudden change.
    Illustrations on the decision boundaries of PGDAT before/after an epoch. 
    Each subfigure contains the decision boundary illustration before (in light-colored) and after (in dark-colored) the adversarial training. 
    }
    \label{fig:PGDAT decision boundary}
\end{figure*}
% \vspace{2em}

==> Figure/PIAT_VIT.tex <==
\begin{table}[t]
\caption{The clean and robust accuracy (\%) of adversarial training methods using ViTs on CIFAR10 dataset. Note that ‘B’ denotes base, ‘S’ denotes ‘small’. The best result in each column is in \textbf{bold}.}
\label{tab:PIAT_ViT}
\begin{center}
\begin{small}
\resizebox{\columnwidth}{!}
{
\begin{tabular}{ccccc}
\toprule
Model& Method &Clean& PGD20& AA\\
\midrule
\multirow{9}{*}{ConViT-B}
  &PGD-AT & 61.47&38.64&34.07\\
  &A\&P &85.21&53.25&49.01\\
  &PIAT+A\&P &\textbf{87.50}&\textbf{56.25}&\textbf{51.86}\\
  \cmidrule(lr){2-5}
    &TRADES& 82.75&52.77&49.61\\
  &A\&P&83.51&53.21&50.11\\
  &PIAT+A\&P&\textbf{86.03}&\textbf{55.88}&\textbf{52.35}\\
  \cmidrule(lr){2-5}
    &MART  &63.61&42.51&37.08\\
  &A\&P&80.32&53.11&48.35\\
  &PIAT+A\&P&\textbf{81.20}&\textbf{56.17}&\textbf{51.13}\\
\midrule
\multirow{9}{*}{ViT-B}
  &PGD-AT  & 83.07&52.93&48.99\\
  &A\&P&84.64&53.44&49.67\\
  &PIAT+A\&P&\textbf{87.83}&\textbf{56.34}&\textbf{52.27}\\
  \cmidrule(lr){2-5}
    &TRADES  &83.45&53.07&49.76\\
  &A\&P&83.91&53.52&50.56\\
  &PIAT+A\&P&\textbf{87.09}&\textbf{55.97}&\textbf{52.57}\\
  \cmidrule(lr){2-5}
    &MART&77.05&52.99&47.95\\
  &A\&P&78.75&53.51&49.01\\
  &PIAT+A\&P&\textbf{82.23}&\textbf{55.94}&\textbf{51.03}\\
\midrule
\multirow{9}{*}{DeiT-S}
  &PGD-AT  & 81.36&47.94&47.28\\
  &A\&P &83.08&52.28&47.92\\
  &PIAT+A\&P&\textbf{83.22}&\textbf{53.55}&\textbf{49.31}\\
  \cmidrule(lr){2-5}
    &TRADES &82.32&52.52&49.07\\
  &A\&P&82.81&52.74&49.40\\
  &PIAT+A\&P&\textbf{83.43}&\textbf{53.31}&\textbf{50.10}\\
  \cmidrule(lr){2-5}
    &MART & 76.77&52.06&47.06\\
  &A\&P&78.43&52.98&47.94\\
  &PIAT+A\&P&\textbf{78.39}&\textbf{53.83}&\textbf{48.97}\\
  \bottomrule
\end{tabular}
}
\end{small}
\end{center}
\centering
\end{table}

==> Figure/PIAT_WRN.tex <==
\begin{table}[t]
\caption{The clean and robust accuracy (\%) of our methods (PIAT+NMSE) and defense baselines using WRN-32-10 model on CIFAR10 and CIFAR100 datasets. 
% The best result in each column is in \textbf{bold}.
}
\label{tab:PIAT_WRN}
\begin{center}
\begin{small}
% \begin{sc}
\resizebox{\columnwidth}{!}
{
\begin{tabular}{ccccc}
\toprule
Dataset& Method &Clean& PGD20& AA\\
\midrule
\multirow{7}{*}{CIFAR10} 
  &PGD-AT  & 86.87&48.77&47.78\\
  &ALP &84.18&53.55&49.68\\
  &TRADES & 82.13&55.14&50.38\\
  &MART&81.57&56.44&49.58\\
  &MAIL&84.96&52.58&47.26\\
  &Generalist&\textbf{91.03}&56.88&52.91\\
\cmidrule(lr){2-5}
  &\textbf{\name+NMSE}&85.04&\textbf{58.04}&\textbf{53.83}\\
  \midrule
  \multirow{7}{*}{CIFAR100}
  &PGD-AT&59.30&28.13&23.99\\
  &ALP &58.11&28.59&24.45\\
  &TRADES&57.99&31.97&26.76\\
  &MART&55.19&31.16&26.46\\
  &MAIL&58.04&29.50&23.97\\
  &Generalist&\textbf{64.62}&33.77&28.94\\
\cmidrule(lr){2-5}
  &\textbf{\name+NMSE}& 61.04&\textbf{35.15}&\textbf{30.07}\\
  \bottomrule
\end{tabular}
}
\end{small}
\end{center}
\centering
\end{table}

==> Figure/PIAT_main_result.tex <==
\begin{table*}[t]
\caption{Comparison of our methods using ResNet18 model trained on CIFAR10, CIFAR100 and SVHN datasets with other adversarial training baseline methods under various adversarial attacks. We report the both natural accuracy (\%) and robust accuracy (\%). The best result in each column is in \textbf{bold}.}
% \linespread{1.25}
\label{table 1: main_result}
\begin{center}
\begin{small}
\begin{tabular}{ccccccccccccc}
\toprule
\multirow{2}{*}{Method} &
  \multicolumn{4}{c}{CIFAR10} &
  \multicolumn{4}{c}{CIFAR100} &
  \multicolumn{4}{c}{SVHN}\\ \cmidrule(lr){2-5}\cmidrule(lr){6-9}\cmidrule(lr){10-13}
  &Natural& PGD20& CW& AA& Natural& PGD20 &CW& AA
  &Natural& PGD20 &CW& AA\\
  \midrule
  PGD-AT~\cite{PGDAT}    &84.28& 50.29& 49.31&46.33& 58.48& 28.36&27.06&23.85&\textbf{93.85}& 59.01&48.66&43.02\\
  ALP~\cite{ALP} &79.74&52.37&49.60&46.13&57.29&28.12&26.84&23.57&92.54&59.13&52.22&45.67\\
  TRADES~\cite{TRADES}    & 82.39 & 53.60& 50.90&48.04&57.98& 29.90&26.14&23.91 & 90.88& 59.50&52.76&46.59 \\
  MART~\cite{MART}     & 81.91& 53.70&49.35&47.45&55.26&30.10&26.00&23.77&90.84&57.70&52.95&46.98\\
  MAIL~\cite{MAIL} &82.65&51.15&48.88&45.16&58.73&27.99&26.28&22.50&90.15&57.47&52.78&46.26\\
  Generalist~\cite{Generalist}& \textbf{89.09}&50.01&50.04&46.07&\textbf{61.97}&29.48&27.77&23.96&92.88&60.21&54.97&49.12 \\
  \midrule
  \textbf{\name+NMSE}    &80.96& \textbf{53.74}&\textbf{51.72}&\textbf{48.80}&56.34&\textbf{31.11}&\textbf{28.45}&\textbf{25.79}& 91.70& \textbf{61.21}&\textbf{55.88}&\textbf{51.29}    \\
\bottomrule
\end{tabular}
\end{small}
\end{center}
\centering
\end{table*}

==> Figure/PIAT_other_method_WRN.tex <==
\begin{table}[t]
\caption{The clean and robust accuracy (\%) of \name framework combined with various adversarial training methods on CIFAR10 dataset with WRN-32-10 model.}
\label{tab:PIAT_WRN_AT}
\begin{center}
\begin{small}
\resizebox{\columnwidth}{!}
{
\begin{tabular}{ccccc}
\toprule
Dataset& Method &Clean& PGD20& AA\\
\midrule
\multirow{10}{*}{CIFAR10} 
  &PGD-AT & \textbf{86.87}&48.77&47.78   \\
  &\textbf{\name}& 85.56&\textbf{52.80}&\textbf{48.35}\\
  \cmidrule(lr){2-5} 
  &ALP &\textbf{84.18}&53.55&49.68\\
  &\textbf{\name}+ALP&83.35&\textbf{57.71}&\textbf{52.35}\\
    \cmidrule(lr){2-5}
  &TRADES & \textbf{82.13}&55.14&50.38\\
  &\textbf{\name}+TRADES&82.08&\textbf{58.93}&\textbf{53.73}\\
  \cmidrule(lr){2-5} 
  &MART&\textbf{81.57}&56.44&49.58\\
  &\textbf{\name}+MART&79.88&\textbf{59.51}&\textbf{52.84}\\
  \cmidrule(lr){2-5} 
  &MAIL&\textbf{84.96}&52.58&47.26\\
  &\textbf{\name}+MAIL&84.24&\textbf{57.53}&\textbf{52.22}\\
  % \midrule
  % \multirow{10}{*}{CIFAR100} 
  % &PGD-AT&59.30&28.13&23.99   \\
  % &\textbf{\name}&\textbf{60.09}&\textbf{34.46}&\textbf{29.47}\\
  % \cmidrule(lr){2-5} 
  % &ALP &58.11&28.59&24.45\\
  % &\textbf{\name}+ALP&\textbf{59.25}&\textbf{34.04}&\textbf{28.94}\\
  % \cmidrule(lr){2-5} 
  % &TRADES&57.99&31.97&26.76\\
  % &\textbf{\name}+TRADES& \textbf{59.78}&\textbf{34.52}&\textbf{29.25}\\
  % \cmidrule(lr){2-5} 
  % &MART&\textbf{55.19}&31.16&26.46\\
  % &\textbf{\name}+MART& 54.32&\textbf{34.87}&\textbf{28.79}\\
  % \cmidrule(lr){2-5} 
  % &MAIL&58.04&29.50&23.97\\
  % &\textbf{\name}+MAIL&\textbf{58.52}&\textbf{33.65}&\textbf{28.00}\\
  \bottomrule
\end{tabular}
}
\end{small}
\end{center}
\centering
\end{table}

==> Figure/decision_boundary_comparision.tex <==
\begin{figure*}[h]
    \centering
    \subfigure[%The decision boundary of PGD-AT 
    From 26\(^{th}\) to 27\(^{th}\) epoch for PGD-AT\label{PGDAT decision boundary}]{
    \includegraphics[width=0.42\textwidth]{Figure/Decision Boundary 26-27.pdf}}
    \subfigure[%The decision boundary of PIAT 
    From 24\(^{th}\) to 25\(^{th}\) epoch for PIAT\label{PIAT decision boundary}]{
    \includegraphics[width=0.42\textwidth]{Figure/PIAT_decision_boundary24-25.pdf}}
    \caption{%The differences of 
    Illustrations on the decision boundaries of PGD-AT or PIAT before/after an epoch. 
    Each subfigure contains the decision boundary illustration before (in light-colored) and after (in dark-colored) the adversarial training. 
    %The light-colored points and decision boundaries represent the state before adversarial training, while the dark-colored points and decision boundaries represent the state after adversarial training.
    }
    \label{fig:Accuracy and Robustness}
\end{figure*}

==> Figure/mitigate_overfitting.tex <==
\begin{table*}[t]
\caption{The natural accuracy (\%) and robust accuracy (\%) of our methods using ResNet18 model trained on CIFAR10 and CIFAR100 with other adversarial training baseline methods under various adversarial attacks. The best result in each column is in \textbf{bold}.}
% \linespread{1.25}
\label{table: mitigating all}
\begin{center}
\begin{small}
\begin{tabular}{ccccccccccccc}
\toprule
\multirow{2}{*}{Dataset} & \multirow{2}{*}{Method} &
  \multicolumn{4}{c}{\textbf{Best Checkpoint}} &
  \multicolumn{4}{c}{\textbf{Last Checkpoint}}\\ \cmidrule(lr){3-6} \cmidrule(lr){7-10}
  &&Natural& PGD20& CW& AA& Natural& PGD20 &CW& AA\\
  \midrule
  \multirow{7}{*}{CIFAR10}
  &PGD-AT~\cite{PGDAT}    &84.28& 50.29& 49.31&46.33&85.62&45.86&43.25&41.36\\
  &ALP~\cite{ALP} &79.74&52.37&49.60&46.13&81.45&48.62&43.87&41.88\\
  &TRADES~\cite{TRADES}    & 82.39 & 53.60& 50.90&48.04&83.04&50.74&49.04&46.80 \\
  &MART~\cite{MART}     & 81.91& 53.70&49.35&47.45&83.99&48.63&43.92&42.01\\
  &MAIL~\cite{MAIL} &82.65&51.15&48.88&45.16&85.17&47.14&44.38&43.02\\
  &Generalist~\cite{Generalist}& \textbf{89.09}&50.01&50.04&46.07&\textbf{89.53}&45.04&45.62&42.60 \\
  \cmidrule(lr){2-10}
  &\textbf{\name+NMSE}    &80.96& \textbf{53.74}&\textbf{51.72}&\textbf{48.80}&82.84&\textbf{52.81}&\textbf{50.49}&\textbf{47.97}    \\
  \midrule
  \multirow{2}{*}{Dataset} & \multirow{2}{*}{Method} &
  \multicolumn{4}{c}{Best Checkpoint} &
  \multicolumn{4}{c}{Last Checkpoint}\\ \cmidrule(lr){3-6} \cmidrule(lr){7-10}
  &&Natural& PGD20& CW& AA& Natural& PGD20 &CW& AA\\
  \midrule
  \multirow{7}{*}{CIFAR100}
  &PGD-AT~\cite{PGDAT}    & 58.48& 28.36&27.06&23.85&58.53&21.72&21.12&19.55\\
  &ALP~\cite{ALP} &57.29&28.12&26.84&23.57&58.65&24.66&22.17&20.49\\
  &TRADES~\cite{TRADES}   &57.98& 29.90&26.14&23.91&56.32&27.70&24.53&22.70 \\
  &MART~\cite{MART}     &55.26&30.10&26.00&23.77&57.77&25.96&23.79&22.35\\
  &MAIL~\cite{MAIL} &58.73&27.99&26.28&22.50&59.00&24.69&23.37&21.86\\
  &Generalist~\cite{Generalist} &\textbf{61.97}&29.48&27.77&23.96&\textbf{67.25}&21.90&21.31&15.61 \\
  \cmidrule(lr){2-10}
  &\textbf{\name+NMSE}    &56.34&\textbf{31.11}&\textbf{28.45}&\textbf{25.79}&56.16&\textbf{30.87}&\textbf{27.76}&\textbf{25.13}    \\
\bottomrule
\end{tabular}
\end{small}
\end{center}
\centering
\end{table*}

==> Figure/mitigating_all.tex <==
\begin{table*}[t]
\caption{The clean and robust accuracy (\%) of our methods (PIAT+NMSE) and defense baselines using ResNet18 model trained on CIFAR10, CIFAR100 and SVHN datasets under various adversarial attacks. We report the results of the best checkpoint according to the highest robust accuracy under PGD20 attack and the final checkpoint. The best result among defense methods in each column is in \textbf{bold}.}
% \linespread{1.25}
\label{table: mitigating all}
\begin{center}
\begin{small}
\begin{tabular}{cccccccccccccc}
\toprule
\multirow{2}{*}{Dataset} & \multirow{2}{*}{Method} &
  \multicolumn{3}{c}{Clean} &
  \multicolumn{3}{c}{PGD20} &
  \multicolumn{3}{c}{CW} &
  \multicolumn{3}{c}{AA}
  \\ \cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11} \cmidrule(lr){12-14}
&&Best&Final&Diff&Best&Final&Diff&Best&Final&Diff&Best&Final&Diff\\
  \midrule
  \multirow{7}{*}{CIFAR10}
  &PGD-AT   
  &84.28&85.62&-1.34&50.29&45.86&~4.43&49.31&43.25&~6.06&46.33&41.36&~4.97\\
  &ALP
  &79.74&81.45&-1.71&52.37&48.62&3.75&49.60&43.87&~5.73&46.13&41.88&~4.25\\
  &TRADES 
   & 82.39&83.04&-0.65& 53.60&50.74&~2.86& 50.90&49.04&~1.86&48.04&46.80&~1.24\\
  &MART  
  &81.91&83.99&-2.08&53.70&48.63&~5.07&49.35&44.92&~4.43&47.45&43.65&~3.80\\
  &MAIL
  &82.65&85.17&-2.49&51.15&47.14&~4.01&48.88&44.38&~4.50&45.16&43.02&~2.14\\
  &Generalist
  & \textbf{89.09}&\textbf{89.53}&\textbf{-0.52}&50.01&45.04&~4.97&50.04&45.62&~4.42&46.07&42.60&~3.47\\
  \cmidrule(lr){2-14}
  &\textbf{\name+NMSE}    
  &80.96&82.84&-1.88&\textbf{53.74}&\textbf{52.81}&\textbf{~0.93}&\textbf{51.72}&\textbf{50.49}&\textbf{~1.23}&\textbf{48.80}&\textbf{47.97}&\textbf{~0.83}\\
  \midrule
  \multirow{7}{*}{CIFAR100}
  &PGD-AT   
  & 58.48&58.53&\textbf{-0.05}& 28.36&21.72&~6.64&27.06&21.12&~5.94&23.85&19.55&~4.30\\
  &ALP
  &57.29&58.65&-1.36&28.12&24.66&~3.46&26.84&22.17&~4.67&23.57&20.49&~3.08\\
  &TRADES 
  &56.71&56.32&-0.39& 29.19&27.70&~1.49&26.05&24.53&~1.52&23.91&22.70&~1.21 \\
  &MART 
  &55.26&57.77&-2.51&30.10&25.96&~4.14&26.30&23.79&~2.51&24.13&22.35&~1.78\\
  &MAIL 
  &58.73&59.00&-0.27&27.99&24.69&~3.30&26.28&23.37&~2.91&22.50&20.86&~1.64\\
  &Generalist
  &\textbf{61.97}&\textbf{67.25}&~5.28&29.48&21.90&~7.58&27.77&21.31&6.46&23.96&15.61&~8.35\\
  \cmidrule(lr){2-14}
  &\textbf{\name+NMSE}    
  &56.04&57.16&-1.12&\textbf{31.45}&\textbf{30.87}&\textbf{~0.58}&\textbf{28.74}&\textbf{27.76}&\textbf{~1.02}&\textbf{26.09}&\textbf{25.13}&\textbf{~0.96}\\
  \midrule
    \multirow{7}{*}{SVHN}
  &PGD-AT  
&\textbf{93.85}&94.33&-0.48& 59.01&52.35&~6.66&48.66&44.13&~4.53&43.02&38.66&~4.36\\
  &ALP &92.54&93.67&-1.13&59.13&55.12&~5.01&52.22&48.53&~3.69&45.67&42.41&~3.26
\\
  &TRADES   & 90.88&91.34&\textbf{-0.46}&59.50&57.04&~2.46&52.76&50.42&~2.34&46.59&44.87&~1.72
\\
  &MART &90.84&92.95&~2.11&57.70&54.29&~3.41&52.95&50.09&~2.86&46.98&43.75&~3.23
\\
  &MAIL &90.15&93.69&-3.54&57.47&54.60&~3.14&52.78&49.73&~3.05&46.26&41.24&~5.02
\\
  &Generalist&92.88&\textbf{96.83}&-3.95&60.21&42.10&18.11&54.97&43.36&11.61&49.12&29.26&19.86
\\
  \cmidrule(lr){2-14}
  &\textbf{\name+NMSE}  &91.70&93.07&-1.37& \textbf{61.21}&\textbf{59.84}&\textbf{~1.37}&\textbf{55.88}&\textbf{54.45}&\textbf{~1.43}&\textbf{51.29}&\textbf{49.82}&\textbf{~1.47}
\\
\bottomrule
% \vspace{-0.4cm}
\end{tabular}
\end{small}
\end{center}
\centering
\end{table*}

==> Tab/PIAT_main_result.tex <==
\begin{table*}[t]
\caption{Comparison of our methods using ResNet18 model trained on CIFAR10, CIFAR100 and SVHN datasets with other adversarial training baseline methods under various adversarial attacks. We report the both natural accuracy (\%) and robust accuracy (\%). The best result in each column is in \textbf{bold}.}
% \linespread{1.25}
\label{table 1: main_result}
\begin{center}
\begin{small}
\begin{tabular}{ccccccccccccc}
\toprule
\multirow{2}{*}{Method} &
  \multicolumn{4}{c}{CIFAR10} &
  \multicolumn{4}{c}{CIFAR100} &
  \multicolumn{4}{c}{SVHN}\\ \cmidrule(lr){2-5}\cmidrule(lr){6-9}\cmidrule(lr){10-13}
  &Natural& PGD20& CW& AA& Natural& PGD20 &CW& AA
  &Natural& PGD20 &CW& AA\\
  \midrule
  PGD-AT~\cite{PGDAT}    &84.28& 50.29& 49.31&46.33& 58.48& 28.36&27.06&23.85&\textbf{93.85}& 59.01&48.66&43.02\\
  ALP~\cite{ALP} &79.74&52.37&49.60&46.13&57.29&28.12&26.84&23.57&92.54&59.13&52.22&45.67\\
  TRADES~\cite{TRADES}    & 82.39 & 53.60& 50.90&48.04&57.98& 29.90&26.14&23.91 & 90.88& 59.50&52.76&46.59 \\
  MART~\cite{MART}     & 81.91& 53.70&49.35&47.45&55.26&30.10&26.00&23.77&90.84&57.70&52.95&46.98\\
  MAIL~\cite{MAIL} &82.65&51.15&48.88&45.16&58.73&27.99&26.28&22.50&90.15&57.47&52.78&46.26\\
  Generalist~\cite{Generalist}& \textbf{89.09}&50.01&50.04&46.07&\textbf{61.97}&29.48&27.77&23.96&92.88&60.21&54.97&49.12 \\
  \midrule
  \textbf{\name+NMSE}    &80.96& \textbf{53.74}&\textbf{51.72}&\textbf{48.80}&56.34&\textbf{31.11}&\textbf{28.45}&\textbf{25.79}& 91.70& \textbf{61.21}&\textbf{55.88}&\textbf{51.29}    \\
\bottomrule
\end{tabular}
\end{small}
\end{center}
\centering
\end{table*}

==> Tab/mitigate_overfitting.tex <==
\begin{table*}[t]
\caption{The natural accuracy (\%) and robust accuracy (\%) of our methods using ResNet18 model trained on CIFAR10 and CIFAR100 with other adversarial training baseline methods under various adversarial attacks. The best result in each column is in \textbf{bold}.}
% \linespread{1.25}
\label{table: mitigating all}
\begin{center}
\begin{small}
\begin{tabular}{ccccccccccccc}
\toprule
\multirow{2}{*}{Dataset} & \multirow{2}{*}{Method} &
  \multicolumn{4}{c}{\textbf{Best Checkpoint}} &
  \multicolumn{4}{c}{\textbf{Last Checkpoint}}\\ \cmidrule(lr){3-6} \cmidrule(lr){7-10}
  &&Natural& PGD20& CW& AA& Natural& PGD20 &CW& AA\\
  \midrule
  \multirow{7}{*}{CIFAR10}
  &PGD-AT~\cite{PGDAT}    &84.28& 50.29& 49.31&46.33&85.62&45.86&43.25&41.36\\
  &ALP~\cite{ALP} &79.74&52.37&49.60&46.13&81.45&48.62&43.87&41.88\\
  &TRADES~\cite{TRADES}    & 82.39 & 53.60& 50.90&48.04&83.04&50.74&49.04&46.80 \\
  &MART~\cite{MART}     & 81.91& 53.70&49.35&47.45&83.99&48.63&43.92&42.01\\
  &MAIL~\cite{MAIL} &82.65&51.15&48.88&45.16&85.17&47.14&44.38&43.02\\
  &Generalist~\cite{Generalist}& \textbf{89.09}&50.01&50.04&46.07&\textbf{89.53}&45.04&45.62&42.60 \\
  \cmidrule(lr){2-10}
  &\textbf{\name+NMSE}    &80.96& \textbf{53.74}&\textbf{51.72}&\textbf{48.80}&82.84&\textbf{52.81}&\textbf{50.49}&\textbf{47.97}    \\
  \midrule
  \multirow{2}{*}{Dataset} & \multirow{2}{*}{Method} &
  \multicolumn{4}{c}{Best Checkpoint} &
  \multicolumn{4}{c}{Last Checkpoint}\\ \cmidrule(lr){3-6} \cmidrule(lr){7-10}
  &&Natural& PGD20& CW& AA& Natural& PGD20 &CW& AA\\
  \midrule
  \multirow{7}{*}{CIFAR100}
  &PGD-AT~\cite{PGDAT}    & 58.48& 28.36&27.06&23.85&58.53&21.72&21.12&19.55\\
  &ALP~\cite{ALP} &57.29&28.12&26.84&23.57&58.65&24.66&22.17&20.49\\
  &TRADES~\cite{TRADES}   &57.98& 29.90&26.14&23.91&56.32&27.70&24.53&22.70 \\
  &MART~\cite{MART}     &55.26&30.10&26.00&23.77&57.77&25.96&23.79&22.35\\
  &MAIL~\cite{MAIL} &58.73&27.99&26.28&22.50&59.00&24.69&23.37&21.86\\
  &Generalist~\cite{Generalist} &\textbf{61.97}&29.48&27.77&23.96&\textbf{67.25}&21.90&21.31&15.61 \\
  \cmidrule(lr){2-10}
  &\textbf{\name+NMSE}    &56.34&\textbf{31.11}&\textbf{28.45}&\textbf{25.79}&56.16&\textbf{30.87}&\textbf{27.76}&\textbf{25.13}    \\
\bottomrule
\end{tabular}
\end{small}
\end{center}
\centering
\end{table*}
